Do "True" and "False" Add Up to One? Complement Consistency in LLM-Agent Opinion Simulations

In LLM-agent opinion simulations, each agent reports the probability that a claim is true after seeing its own previous probability and the probabilities reported by its neighbors, and that number becomes its state in the next round. If the number describes the agent's position rather than the sentence it was shown, then rewriting the claim as its complement and replacing every probability p with 1 - p should return the complementary answer, so the two reports should sum to one. We test this with three small open models: Qwen3-4B, Llama-3.2-3B and Gemma-3-4B. On 2,304 agent states taken from a running network simulation, Qwen's paired reports sum to 1.18 on average, and on 48 real fact-checking claims from AVeriTeC they again exceed one. A controlled benchmark of 24 worlds, each with exactly two possible outcomes, shows the same failure in all three models. The discrepancy is two to ten times larger than the change produced by a same-meaning paraphrase, and it persists under repeated sampling and across peer group sizes and report strengths. When the reports are fed back into two populations that start from complementary states, the populations do not remain mirror images: their divergence is positive after five rounds for every model. Averaging each answer with the complement of its paired answer restores consistency by construction and lowers Brier loss averaged over the two wordings, but at the final round it beats the better of the two original wordings for only one of the three models. A schedule-by-targeting experiment on the same model gives a small, stable interaction because such sweeps keep the claim wording fixed. Consistency under rewording therefore needs its own test before simulated probabilities are read as beliefs

==> figures/world-panels.tex <==
\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S9_world_paths_qwen_absent.pdf}
\caption{All six worlds and both placements for Qwen, evidence absent. Columns show trajectory discrepancy, common-coordinate population mean, and within-population variance. Solid/dashed curves distinguish placements; filled/open markers distinguish the original and converted complementary paths in the mean/variance panels. Discrepancy and means use [0,1]; variance uses [0,0.26]. All five update rounds are shown.}\label{fig:appendix-S9_world_paths_qwen_absent}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S9_world_paths_qwen_visible.pdf}
\caption{All six worlds and both placements for Qwen, evidence visible. Columns show trajectory discrepancy, common-coordinate population mean, and within-population variance. Solid/dashed curves distinguish placements; filled/open markers distinguish the original and converted complementary paths in the mean/variance panels. Discrepancy and means use [0,1]; variance uses [0,0.26]. All five update rounds are shown.}\label{fig:appendix-S9_world_paths_qwen_visible}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S9_world_paths_llama_absent.pdf}
\caption{All six worlds and both placements for Llama, evidence absent. Columns show trajectory discrepancy, common-coordinate population mean, and within-population variance. Solid/dashed curves distinguish placements; filled/open markers distinguish the original and converted complementary paths in the mean/variance panels. Discrepancy and means use [0,1]; variance uses [0,0.26]. All five update rounds are shown.}\label{fig:appendix-S9_world_paths_llama_absent}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S9_world_paths_llama_visible.pdf}
\caption{All six worlds and both placements for Llama, evidence visible. Columns show trajectory discrepancy, common-coordinate population mean, and within-population variance. Solid/dashed curves distinguish placements; filled/open markers distinguish the original and converted complementary paths in the mean/variance panels. Discrepancy and means use [0,1]; variance uses [0,0.26]. All five update rounds are shown.}\label{fig:appendix-S9_world_paths_llama_visible}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S9_world_paths_gemma_absent.pdf}
\caption{All six worlds and both placements for Gemma, evidence absent. Columns show trajectory discrepancy, common-coordinate population mean, and within-population variance. Solid/dashed curves distinguish placements; filled/open markers distinguish the original and converted complementary paths in the mean/variance panels. Discrepancy and means use [0,1]; variance uses [0,0.26]. All five update rounds are shown.}\label{fig:appendix-S9_world_paths_gemma_absent}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S9_world_paths_gemma_visible.pdf}
\caption{All six worlds and both placements for Gemma, evidence visible. Columns show trajectory discrepancy, common-coordinate population mean, and within-population variance. Solid/dashed curves distinguish placements; filled/open markers distinguish the original and converted complementary paths in the mean/variance panels. Discrepancy and means use [0,1]; variance uses [0,0.26]. All five update rounds are shown.}\label{fig:appendix-S9_world_paths_gemma_visible}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S10_world_repair_qwen.pdf}
\caption{Final and time-mean visible Brier changes for all six worlds under Qwen. Each active arm is compared against baseline x, baseline z and their equal-loss average in separate columns. Active-arm values average orientation losses, except symmetrization, which is one coupled process. Positive values expose harm relative to the stated reference. All arms/worlds are shown; identical greedy averaging and zero changes remain visible. Corrected Llama comparisons use its date-matched fresh baseline, with different-session limitations.}\label{fig:appendix-S10_world_repair_qwen}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S10_world_repair_llama.pdf}
\caption{Final and time-mean visible Brier changes for all six worlds under Llama. Each active arm is compared against baseline x, baseline z and their equal-loss average in separate columns. Active-arm values average orientation losses, except symmetrization, which is one coupled process. Positive values expose harm relative to the stated reference. All arms/worlds are shown; identical greedy averaging and zero changes remain visible. Corrected Llama comparisons use its date-matched fresh baseline, with different-session limitations.}\label{fig:appendix-S10_world_repair_llama}\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/S10_world_repair_gemma.pdf}
\caption{Final and time-mean visible Brier changes for all six worlds under Gemma. Each active arm is compared against baseline x, baseline z and their equal-loss average in separate columns. Active-arm values average orientation losses, except symmetrization, which is one coupled process. Positive values expose harm relative to the stated reference. All arms/worlds are shown; identical greedy averaging and zero changes remain visible. Corrected Llama comparisons use its date-matched fresh baseline, with different-session limitations.}\label{fig:appendix-S10_world_repair_gemma}\end{figure*}


==> final_fixes.tex <==
% =====================================================================
% final_fixes.tex  --  copy-paste replacements (not a compilable file)
% Search for the first few words of each FIND string; if your file
% differs slightly from the PDF text, match on those words.
% =====================================================================

% ---------------------------------------------------------------------
% 1. ABSTRACT: two sentences overreach
% ---------------------------------------------------------------------
% FIND:    A schedule-by-targeting experiment on the same model gives a small,
%          stable interaction because such sweeps keep the claim wording fixed.
% REPLACE: A conventional schedule-by-targeting sweep on the same model leaves
%          its interaction statistically unresolved and cannot detect the
%          inconsistency, because it keeps the claim wording fixed.
%
% FIND:    but it does not always beat the better of the two original wordings.
% REPLACE: but at the final round it beats the better of the two original
%          wordings for only one of the three models.
%
% CHECK:   "two to ten times larger". From Figure 3 I read ratios of roughly
%          2.4 (Llama, visible) to 9.5 (Gemma, absent). Compute them from the
%          data and write the exact range.

% ---------------------------------------------------------------------
% 2. INTRODUCTION
% ---------------------------------------------------------------------
% FIND:    The question admits a direct test (Figure 1).
% REPLACE: The question can be tested directly (Figure 1).
%
% Figure 1 currently shows the schedule sweep, not the complement test. Swap
% in the red/blue token figure (one world, original vs complementary
% description, four peers) and move the sweep schematic to the appendix or drop it.
%
% FIND:    "Our contribution is an evaluation of complete social update requests
%          ... while keeping factual accuracy and computational cost explicit."
% REPLACE:
We make three contributions. First, we define a complement-consistency test
for the update step of an LLM-agent simulation and show that three small open
models fail it on states from a running simulation, on real fact-checking
claims, and on a controlled benchmark in which every world has exactly two
outcomes. Second, we show that the failure exceeds sensitivity to a
same-meaning paraphrase, persists under repeated sampling and across peer
counts and report strengths, and carries into later rounds when reports are
fed back into the simulation. Third, we evaluate averaging each report with
the complement of its paired report, which restores consistency by
construction, and show that its effect on factual loss under feedback depends
on the model.
%
% Then DELETE the paragraph "The studies yield three connected findings ..."
% (it repeats the abstract).

% ---------------------------------------------------------------------
% 3. RELATED WORK
% ---------------------------------------------------------------------
% FIND:    in trained artificial-language models
% REPLACE: in language models
%
% ADD one paragraph (keys sclar2024 and tjuatja2024 are in your CIKM references.bib):
\paragraph{Wording and response bias.}
Meaning-preserving changes to prompt wording and format can move model
outputs by large margins \citep{sclar2024}, and models respond to
acquiescence-style manipulations of survey items differently from people
\citep{tjuatja2024}. Our test differs in that one transformation changes the
claim, the agent's probability and every peer report together, so the
correct response is fixed by arithmetic.
%
% references.bib: Tramer -> Tram{\`e}r in the Fluri et al. and Paleka et al. entries.

% ---------------------------------------------------------------------
% 4. NOTATION CLASHES (each symbol must mean one thing)
% ---------------------------------------------------------------------
% q_{o,p} (paraphrase) clashes with the prior p      -> q_o^{\mathrm{base}}, q_o^{\mathrm{para}} (Eq. 5)
% b = world seed (Eq. 14) clashes with b = F(T(s))   -> world seed: w
% pi = targeting policy clashes with pi = joint law  -> joint law of draws: \gamma (Eqs. 7, 8)
% R_src (Eq. 19) clashes with R(s) (Eq. 24)          -> goes away if Section 8 below is cut
% Eqs. 24-26: replace q with q_0 and b with q_1 (matches Figure 1 and the new repair figure):
%   R(s) = (q_0 + 1 - q_1)/2,   delta(s) = q_0 + q_1 - 1

% ---------------------------------------------------------------------
% 5. LEFTOVER CODEBASE LANGUAGE (find -> replace)
% ---------------------------------------------------------------------
% "committed updates" (Design; Table 2 caption; Appendix D)       -> "agent updates"
% "encountered" (Intro; Results heading; "encountered states" x2) -> "simulation states"
%       heading: "Complement Tests on Simulation States and Real Claims"
% "denoted $A_0$ in the original analysis, is"                    -> "is"
% "The original uncertainty analyses use 10,000 frozen bootstrap resamples." -> "Intervals use 10,000 bootstrap resamples."
% "Cached request reuses and multiple recipients do not become independent resampling units." -> delete
% FIND:    These three studies use the Qwen checkpoint at temperature 0.2, with
%          one recorded report per distinct request. They establish the
%          simulation setting and characterize the elicited requests.
% REPLACE: These three studies use Qwen at temperature 0.2.
% FIND:    and additional checkpoint protocols. The real-claim results and
%          controlled results retain their own estimands and denominators.
% REPLACE: and additional models.
% FIND:    These results characterize stochastic single reports on encountered
%          states and constructed real-claim negations.
% REPLACE: These results concern single stochastic reports from Qwen, on
%          simulation states and on negations we wrote for real claims.
% FIND:    The minimum-adjustment identity gives a mean per-coordinate numerical
%          correction of 0.1630.
% REPLACE: Restoring consistency would require changing each report by
%          $|\delta|/2$, which averages 0.163 (Section on symmetrization).
% FIND:    A single global offset does not describe these recorded pairs.
% REPLACE: No single constant offset describes these pairs.
% FIND:    ... whereas Gemma's increase, so the size of the discrepancy does not
%          rank the models by factual performance.
% REPLACE: ... whereas Gemma's increase. The discrepancy measures consistency,
%          not accuracy, so it does not rank the models by factual performance.
% FIND:    Per-world trajectories, population means and variances appear in the appendix.
% REPLACE: (delete; the appendix has no such figures)
% "Results by family and by world appear in the appendix." -> "Results by family appear in Appendix C."
% "Complete results appear in the appendix."                -> "Complete results appear in Appendix C."
% "The full grid appears in the appendix."                  -> "The full grid appears in Appendix C."
% "...per-world repair differences, appear in the appendix." -> "Both orientations for every arm appear in Appendix C."
% "The appendix gives the full prompts, one filled-in original and complementary pair, and all decoding settings."
%                                                           -> "Appendix A gives the prompts and one filled-in complementary pair; Appendix D gives the decoding settings."
%
% Results heading "Scheduling and Targeting Measure a Different Property"
%                                       -> "A Conventional Sweep Leaves the Interaction Unresolved"
%
% FIND:    The prespecified decision rule does not identify equivalence from this result.
% FIX:     The interval lies inside the +/-0.02 margin, yet the text says the
%          result is not equivalence. State the rule in one sentence, or write
%          "We therefore make no equivalence claim." A reviewer will ask.

% ---------------------------------------------------------------------
% 6. TABLES
% ---------------------------------------------------------------------
% Table 1: columns must be  Model | Quantization | Instruction placed in
%   Qwen3-4B-Instruct-2507 | Q4_K_M  | System message
%   Llama-3.2-3B-Instruct  | Q4_K_M  | System message
%   Gemma-3-4B-IT          | QAT Q4_0 | Start of user message
%   (delete "Logical roles" and the "Native template / matched date / Direct
%   constrained schema" column; they are old pipeline notes)
% Table 2: delete the "Llama baseline rerun" row, or write
%   "Llama baseline rerun | Rerun of the Llama baseline with the date fixed | 960".
%   Move the whole table to the appendix if you need space.
% Table 4: "Real claims: absolute discrepancy 0.3259 - -" -> compute the same
%   claim-within-label bootstrap interval and fill it in.

% ---------------------------------------------------------------------
% 7. FEEDBACK FIGURE: wording that the data do not support
% ---------------------------------------------------------------------
% Figure 4 caption: "Qwen's divergence declines after the first rounds"
%    -> "Qwen's divergence stays roughly flat after the first round"
% Text: "Qwen's divergence falls from its first to its final update"
%    -> "Qwen's divergence stays roughly flat (about 0.23 to 0.28)"
%    (read from the figure; check the exact range in your data)

% ---------------------------------------------------------------------
% 8. CUT FROM THE MAIN TEXT (about 2 pages; main text is now 10 pages)
% ---------------------------------------------------------------------
% - Subsection "Attraction, Accuracy, and Evidence Access" (Eqs. 17-23)
% - Results subsection "Attraction, Accuracy, and Consistency Separate
%   Empirically", Table 5, Table 4 rows R_src and P, Figure 12 and Table 8's P rows
% - In Discussion, replace the paragraph "Consistency and factual utility" with:
Consistency and factual accuracy answer different questions. Symmetrization
improves loss averaged over the two wordings while sometimes underperforming
the better original wording, so assessing a repair requires wording-specific
losses and whole-trajectory outcomes.
% - Table 3 and Figure 2: reduce to one paragraph (numbers: I = 0.0015,
%   interval [-0.0093, 0.0132]) or move to the appendix
% - Table 2: appendix
% - Equations 9-10 (the estimators): appendix
% - The "greedy average" arm and the cost paragraph: one sentence
%   ("Averaging two identical greedy calls reproduces the baseline exactly.")

% ---------------------------------------------------------------------
% 9. RESULTS: add one honest sentence (reviewers will compute it)
% ---------------------------------------------------------------------
% After "...215 of 288 Qwen pairs and 210 of 288 Llama pairs are exactly consistent." add:
So with evidence visible, the average discrepancy for these two models comes
from about a quarter of the pairs, and for Qwen it is concentrated in event
order and set membership (Appendix C); some of that may reflect how hard it is
to verify the complementary description rather than wording alone, which is why
we compare against paraphrase sensitivity.

% ---------------------------------------------------------------------
% 10. APPENDIX
% ---------------------------------------------------------------------
% (a) Prompt boxes are no longer verbatim. The PDF shows "output contract."
%     (the version tag is gone) and the user template has lost the repeated
%     definition lines that the models received. Either restore them or disclose.
%     Replace the first sentence of Appendix A with:
The boxes reproduce the messages sent to the models. Line wrapping differs, and
an internal version identifier that followed ``output contract'' in the first
line of each message is omitted.
%     and restore this line in the user template box, after "Apply output contract.":
%       [The probability definition and scale from the system instruction are repeated here, unchanged.]
%
% (b) Five "Figure ??": the figure files carry different labels. In each file
%     under figures/, set the \label to:
%       appendix-family  -> \label{fig:app-family}
%       appendix-negation -> \label{fig:app-negation}
%       appendix-sampling -> \label{fig:app-sampling}
%       appendix-prompts  -> \label{fig:app-prompts}
%       appendix-peers    -> \label{fig:app-peers}
%     Find them with:  grep -n "label" figures/appendix-*.tex
%
% (c) Captions in Figures 7-12 still contain the old language. Replace with:
% Fig 7 (family):
%   Mean absolute complement discrepancy by structural family (four worlds each) with affirmative descriptions, for each model and evidence condition. Bars at zero are measured values.
% Fig 8 (negation):
%   Change in absolute discrepancy for each world when the complementary description is an explicit negation instead of an affirmative alternative. Negative values mean the negation reduced the discrepancy. Sw: switch, Co: color, Set: membership, Par: parity, Ord: event order, Thr: threshold.
% Fig 9 (sampling):
%   Discrepancy of the mean reports (circles) and mean discrepancy of independently paired draws (diamonds), from 80 draws per request on the six-world subset. Where only a diamond is visible, the two coincide.
% Fig 10 (prompt controls):
%   Change relative to the matched baseline for each prompt control. Left: absolute complement discrepancy (open squares, evidence absent; filled circles, evidence visible). Right: visible Brier loss averaged over orientations. Evidence prose and reordering apply only with visible evidence.
% Fig 11 (peer grid):
%   Mean absolute complement discrepancy by peer count and symmetric report pair. Each cell averages six worlds, two priors and three opposition levels; the outlined cell is the four-peer, 0.2/0.8 setting used in the main tests.
% Fig 12 (dose-response; only if kept):
%   Truth-directed probability on the 48 real claims as the share of peers opposing the initial position increases, averaged over claims and both wordings. Rows: initial position aligned with or opposed to the dataset label. Columns: audience. Error bars are 95% claim-bootstrap intervals; the dotted line marks probability 0.5.
%
% (d) Main Figure 5: delete the two lines printed under the plots inside the
%     image ("Filled circles: ...", "Open triangles: ..."); the caption says it.

% ---------------------------------------------------------------------
% 11. NEW FIGURE (repair mechanism): place at the top of Section "Averaging,
%     Symmetrization, and Utility", before "What the Algebra Guarantees"
% ---------------------------------------------------------------------
\begin{figure*}[t]
\centering
\includegraphics[width=0.92\textwidth]{figures/repair-mechanism.pdf}
\caption{Symmetrization. Left: the same state is described in both
orientations and the model answers each request in a separate call, giving
$q_0$ and $q_1$. Middle: $q_1$ is mapped back to the original orientation as
$1-q_1$ and averaged with $q_0$ to give $R$. The repaired pair $(R,1-R)$ is
complementary by construction, and for this fixed pair the average Brier loss
falls by $\delta^2/4$. Right: repaired reports become the next round's states
and are compared with the unrepaired populations on factual loss and call
cost. The one-step identity does not determine the outcome of this
closed-loop comparison.}
\label{fig:repair-mech}
\end{figure*}
% Cite it in the first sentence of "What the Algebra Guarantees" and in "Closed-Loop Results".
% Edits to the image itself:
%   "Same checkpoint (frozen parameters)"  -> "Same model"
%   "Same evidence  s (fixed state)"       -> "Same evidence" (s is the whole request in the text)
%   q_t, q'_t                              -> x_t, z_t (the populations' symbols in Section 3)
%   delete the bottom banner (the sentence is in the caption)


==> tables/orientations.tex <==
\begin{table*}[t]\centering
\begin{tabular}{@{}llrrrr@{}}\toprule
Protocol & Arm & $L_0(5)$ & $L_1(5)$ & Mean final & Mean rounds\\\midrule
Qwen & Baseline & 0.083 & 0.250 & 0.167 & 0.168\\
Qwen & Reminder & 0.000 & 0.229 & 0.115 & 0.138\\
Qwen & Greedy average & 0.083 & 0.250 & 0.167 & 0.168\\
Qwen & Symmetrization & 0.147 & 0.147 & 0.147 & 0.098\\
\addlinespace
Llama & Baseline & 0.071 & 0.345 & 0.208 & 0.196\\
Llama & Reminder & 0.074 & 0.209 & 0.142 & 0.191\\
Llama & Greedy average & 0.071 & 0.345 & 0.208 & 0.196\\
Llama & Symmetrization & 0.153 & 0.153 & 0.153 & 0.169\\
\addlinespace
Gemma & Baseline & 0.261 & 0.291 & 0.276 & 0.259\\
Gemma & Reminder & 0.247 & 0.334 & 0.290 & 0.268\\
Gemma & Greedy average & 0.261 & 0.291 & 0.276 & 0.259\\
Gemma & Symmetrization & 0.116 & 0.116 & 0.116 & 0.144\\
\addlinespace
\bottomrule\end{tabular}
\caption{Visible-evidence repair utility with both orientations retained. Entries average six worlds at one placement; lower is better. Mean final averages $L_0(5)$ and $L_1(5)$; mean rounds additionally averages rounds 1--5. Symmetrization has a shared complementary display, so its two equal losses are not independent observations. Llama uses the corrected native-date baseline. Three-decimal equality can reflect rounding.}\label{tab:orientations}\end{table*}

==> tables/real-labels.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}llrr@{}}
\toprule
Dataset label & Outcome & Estimate & Pointwise $95\%$ interval\\
\midrule
Supported & Signed discrepancy & 0.3488 & $[0.3016,0.3948]$\\
Supported & Absolute discrepancy & 0.3647 & $[0.3276,0.4042]$\\
Supported & Evidence protection & 0.0100 & $[-0.0822,0.1039]$\\
Refuted & Signed discrepancy & 0.0246 & $[-0.0673,0.1163]$\\
Refuted & Absolute discrepancy & 0.2872 & $[0.2307,0.3469]$\\
Refuted & Evidence protection & 0.0400 & $[-0.0572,0.1323]$\\
\bottomrule
\end{tabular}
\caption{Real-claim results by original dataset label, with within-label claim bootstrap intervals. Small signed discrepancy can coexist with larger absolute discrepancy because opposite signs cancel. The constructed negations are retained as elicited; the controlled study separately fixes exhaustive binary predicates.}\label{tab:real-labels}
\end{table*}

